Constrained Monotonic Neural Networks

Wider adoption of neural networks in many critical domains such as finance and healthcare is being hindered by the need to explain their predictions and to impose additional constraints on them. Monotonicity constraint is one of the most requested properties in real-world scenarios and is the focus of this paper. One of the oldest ways to construct a monotonic fully connected neural network is to constrain signs on its weights. Unfortunately, this construction does not work with popular non-saturated activation functions as it can only approximate convex functions. We show this shortcoming can be fixed by constructing two additional activation functions from a typical unsaturated monotonic activation function and employing each of them on the part of neurons. Our experiments show this approach of building monotonic neural networks has better accuracy when compared to other state-of-the-art methods, while being the simplest one in the sense of having the least number of parameters, and not requiring any modifications to the learning procedure or post-learning steps. Finally, we prove it can approximate any continuous monotone function on a compact subset of $\mathbb{R}^n$.

==> 0_abstract.tex <==
%auto-ignore

\begin{abstract}
Wider adoption of neural networks in many critical domains such as finance and healthcare is being hindered by the need to explain their predictions and to impose additional constraints on them. Monotonicity constraint is one of the most requested properties in real-world scenarios and is the focus of this paper.  
One of the oldest ways to construct a monotonic fully connected neural network is to constrain signs on its weights. Unfortunately, this construction does not work with popular non-saturated activation functions as it can only approximate convex functions. We show this shortcoming can be fixed by constructing two additional activation functions from a typical unsaturated monotonic activation function and employing each of them on the part of neurons. Our experiments show this approach of building monotonic neural networks has better accuracy when compared to other state-of-the-art methods, while being the simplest one in the sense of having the least number of parameters, and not requiring any modifications to the learning procedure or post-learning steps.
Finally, we prove it can approximate any continuous monotone function on a compact subset of $\mathbb{R}^n$.
\end{abstract}

==> 1_introduction.tex <==
%auto-ignore

\section{Introduction} \label{sec:Intro}

Deep Learning has witnessed widespread adoption in many critical real-world domains such as finance, healthcare, etc \citep{LeCun2015}. 
% Predictive models built using deep neural networks have been shown to have high accuracy. 
Incorporating prior knowledge such as monotonicity in trained models helps in improving the performance and generalization ability of the trained models \citep{Mitchell80theneed,dugas2000incorporating}. The introduction of structural biases such as monotonicity makes models also more data-efficient, enabling a leap in predictive power on smaller datasets \citep{velickovic2019phd}.
Apart from the requirements of having models with high accuracy, there is also a need for transparency and interpretability, and monotonicity helps in partially achieving the above requirements \citep{gupta2016monotonic}. 
% this is a bit too abstract, let's make it more concrete.
% Enforcing monotonicity with respect to some input or all the inputs in highly expressive models such as neural networks, would make the models better suitable for real-world adoption. Also, in certain scenarios, it is imperative that the machine learning models are monotonic with respect to some of the inputs because of legal and/or ethical and/or safety concerns.
% Moreover in some machine learning applications such as finance and medicine, monotonicity is a property that the trained models should possess by nature. 
Due to legal, ethical and/or safety concerns, monotonicity of predictive models with respect to some input or all the inputs is required in numerous domains such as financial (house pricing, credit scoring, insurance risk), healthcare (medical diagnosis, patient medication) and legal (criminal sentencing) to list just a few. 
% All other things being equal, a larger house should be deemed more valuable, a bank's clients with higher income should be eligible for a larger loan \citep{sharma2020higher}, and an offender with a longer crime history should be predicted as more likely to commit another crime \citep{Rudin2020Age}, etc.
For example, when using machine learning to predict admission decisions, it may seem unfair to select student X over student Y, if Y has a higher score than X, while all other aspects of the two are identical \cite{liu2020certified}. In another example, one would expect an individual with a higher salary to have a higher loan amount approved, all else being equal \cite{sivaraman2020counterexample}.
A model without such a monotonic property would not, and certainly should not, be trusted by society to provide a basis for such important decisions. 
% However, the monotonicity of deep learning models is not a guaranteed property even when trained on monotonic data, let alone when training on noisy data typically used in practice.
% end rewrite
% Last but not least, enforcing monotonicity in trained models not only help in transparency but also improve generalization by preventing overfitting \cite{dugas2000incorporating}. 

% Although monotonicity is an important and increasingly often even required property, there is no simple or easy method to enforce it. 
Monotonicity has been an active area of research and the existing methods on the subject can be broadly categorized into two types:

\begin{enumerate}
    \item Monotonic architectures by construction: neural architectures guaranteeing monotonicity by construction \citep{archer1993application,sill1997monotonic,daniels2010monotone, milani2016fast, you2017deep}.
    % One of the main problems with these hand-designed monotonic architectures is that they can be very constrained or restrictive and lose out on the expressiveness of non-constrained neural networks. They also tend to be difficult to implement in practice.

    %%% todo:
    % 
    
    
    \item Monotonicity by regularization:  enforcing monotonicity in neural networks during training by employing a modified loss function or a heuristic regularization term \citep{sill1996monotonicity,gupta2019incorporate}.
    %rebuttal
    % However, employing a modified loss function or a regularization term give us no guarantees that the trained model is indeed monotonic. A recent line of research work focuses on verifying/certifying monotonicity of such models \citep{sivaraman2020counterexample, liu2020certified}. These approaches are computationally very expensive and they require multiple retraining cycles to enforce monotonicity.
    
\end{enumerate}
% We give a more detailed account of the existing methods in the next section.

The simplest method to achieve monotonicity by construction is to constrain the weights of the fully connected neural network to have only non-negative (for non-decreasing variables) or only non-positive values (for non-ascending) variables when used in conjunction with a monotonic activation function, a technique known for 30 years \citep{archer1993application}. 
% However, this method does not work well in practice.
When used in conjunction with saturated (bounded) activation functions such as the sigmoid and hyperbolic tangent, these models are difficult to train, i.e. they do not converge to a good solution. On the other hand, when used with non-saturated (unbounded) convex activation functions such as ReLU \citep{nair2010rectified}, the resulting models are always convex \citep{liu2020certified}, severely limiting the applicability of the method in practice.

Our main contribution is a modification of the method above which, in conjunction with non-saturated activation functions, is capable of approximating non-convex functions as well: when the original activation function is used with additional two monotonic activation functions constructed from it in a neural network with constrained weights, it can approximate any monotone continuous functions.

% There are several possible ways to satisfy this condition, with the simplest one using both an activation function $\breve{\rho}$ and its point reflection with respect to point $(0, 0)$ defined as:
% $$
% % \dot{a}(x) = -a(-x)
% \hat{\rho}(x) = -\breve{\rho}(-x)
% $$
% Assuming the original activation function $\breve{\rho}$ is both monotonic and convex, the properties holding for ReLU, ELU, SELU, and Softplus, the proposed modification uses the original activation function $\breve{\rho}$ on a part of the neurons in the network and its point reflection $\hat{\rho}$ on the rest of the neurons.

%rebuttal
% Depending on whether should the resulting model be convex, concave or neither, the part of the neurons using the original activation function is all, nothing or something in between, respectively.

The resulting model is guaranteed to be monotonic, can be used in conjunction with popular convex monotonic non-saturated activation function, doesn't have any additional parameters compared to a non-monotonic fully-connected network for the same task, and can be trained without any additional requirements on the learning procedure. Experimental results show it is exceeding the performance of all other state-of-the-art methods, all while being both simpler (in the number of parameters) and easier to train.

% we don't have such experiments in this paper
% We also discuss other options to construct appropriate activation functions including learnable activation functions such as S-shaped ReLU \citep{jin2016deep} and a novel learnable activation function termed \emph{yet another activation function}. Our experiments show that such construction can result in even higher performance, but with higher variance as they are less stable and more sensitive to random initialization.
 
% Last but not least, we briefly discuss how the method above can be extended to other neural architectures such as convolutional and recurrent. Due to space constraints, we postpone a more thorough experimental account for future work.

% To this end, we build a simple and elegant monotonic fully connected layer that can be used as a drop-in replacement of a fully connected layer in building and training neural networks. Our method can employ the modern activation functions and not only enforce convex monotonicity but also concave monotonicity and even concavo-convex and convexo-concave monotonicities.



% In the light of previous research work on monotonic architectures, the main question we pose to ourselves is-
% \begin{quote}
% Can we construct monotonic architectures that are not restrictive and are more expressive?
% \end{quote}

% To this end, we build a simple and elegant monotonic feedforward dense/fully-connected layer or block that can be directly used to construct generic neural network architectures to enforce monotonicity. 


Our contributions can be summarized as follows:
\begin{enumerate}
    \item A modification to an existing constrained neural network layer enabling it to model arbitrary monotonic function when used with non-saturated monotone convex activation functions such as ReLU, ELU, SELU, and alike.
    
    % \item We prove the monotonicity property of neural architectures using the proposed constricted neural network layer using the ReLU activation function.
    
    % \item We perform extensive ablation studies to show empirically how our proposed monotonic dense layer performs.
    
    \item Experimental comparisons with other recent works showing that the proposed architecture can yield equal or better results than the previous state-of-the-art and with significantly fewer parameters.
    
    %rebuttal
    \item A proof showing that the proposed architecture can approximate any monotone continuous function on a compact subset of $\mathbb{R}^n$ for a large class of non-saturated activation functions.
\end{enumerate}

==> 2_related.tex <==
%auto-ignore

\section{Related work}

% Before dwelling on the methods employed to build monotonic models, we give an overview of activation functions as they form a crucial part of our work. 
% Finally, we discuss universal approximation theorem for different kind of neural architectures.


\subsection{Activation functions}


Right from its inception in perceptron \citep{rosenblatt1958perceptron}, non-linear activation functions have historically been one of the most important components of neural networks. Previously, the saturated functions such as the sigmoid \citep{rumelhart1986learning}, the hyperbolic tangent \citep{neal1992connectionist}, and its variants were the most common choice of activation functions. 
Currently, one of the most important factors for state-of-the-art results accomplished by modern neural networks is the use of non-saturated activation functions. The use of \emph{Rectified Linear Unit} (ReLU) \citep{nair2010rectified, glorot2011deep} as activation function was instrumental in achieving good performance in newer architectures. The ReLU has since become a de facto choice of activation in most practical implementations and continues to be widely used because of its advantages such as simple computation, representational sparsity, and linearity.
%%rebuttal
Later, a number of activation functions were proposed to deal with solving problems of dead neurons and aid in faster convergence \citep{maas2013rectifier}, \citep{clevert2015fast} \citep{he2015delving}, \citep{zheng2015improving},  \citep{hendrycks2016gaussian},  \citep{ramachandran2017swish},  \citep{klambauer2017self}.
%% before rebuttal
% Later, a number of activation functions were proposed to deal with solving problems of dead neurons and aid in faster convergence: \emph{Leaky ReLU} \citep{maas2013rectifier}, \emph{Exponential Linear Unit} (ELU) \citep{clevert2015fast}, \emph{Parametric ReLU} (PReLU)  \citep{he2015delving}, \emph{Softplus} \citep{zheng2015improving}, \emph{Gaussian Error Linear Units} (GELU) \citep{hendrycks2016gaussian}, \emph{Swish} \citep{ramachandran2017swish}, \emph{Scaled Exponential Linear Unit} (SELU) \citep{klambauer2017self} etc.

% Later, small modifications to ReLU activation function termed \emph{Leaky ReLU} \citep{maas2013rectifier} and \emph{Exponential Linear Unit} (ELU) \citep{clevert2015fast} were proposed to address the problem of dead neurons in ReLU. A parametic form of Leaky ReLU termed \emph{Parametric ReLU} (PReLU) was later proposed in \citep{he2015delving}. 
% The authors of \cite{he2015delving} also introduced a better initialization scheme for these rectifier-like activation functions that helped in exploring powerful deep neural architectures and was one of the first works that surpassed the human performance in Imagenet classification task \citep{russakovsky2015imagenet}.

% The major advantages attributed to the use of non-saturated activation functions such as ReLU, Leaky ReLU, ELU and PReLU over the saturated ones such as \emph{sigmoid} and \emph{hyperbolic tangent} are alleviation of the problem of exploding and vanishing gradient and acceleration of the convergence during training \citep{xu2015empirical}.

% The more recent works on activation functions such as \emph{Softplus} \citep{zheng2015improving}, \emph{Gaussian Error Linear Units} (GELU) \citep{hendrycks2016gaussian}, \emph{Swish} \citep{ramachandran2017swish}, \emph{Scaled Exponential Linear Unit} (SELU) \citep{klambauer2017self} etc., have broadly focussed on solving problems of dead ReLU and aid in faster convergence. These activation functions have been shown to provide improved results and hence tend to be useful in practice. 


% ReLU and its variants LeakyReLU, PReLU, ELU, SELU and Softmax have the following important properties for our work: they are non-decreasing, monotonic and convex. Notice that this is not a general rule for activation functions used today, e.g. GELU, Swish are not monotonic and we will not use it in our construction.




The idea of using both the original activation function and its point reflection in the same layer has been proposed in \cite{DBLP:journals/corr/ShangSAL16} where both outputs of ReLU and the negative value of its point reflection were used in the construction of \emph{concatenated ReLU} (CReLU) activation function. The proposed modification outputs two values instead of one and therefore increases the number of parameters. In \cite{Zagoruyko2017diracnets}, the authors propose \emph{negative concatenated ReLU} (NCReLU) flip the sign and use the point reflection directly. 
% Notice that the proposed architectural change could be applied to other non-saturated, monotonic activation functions as well, but with an unknown impact on their performance.
In \cite{DBLP:conf/iclr/EidnesN18}, the authors propose \emph{bipolar ReLU} which consists of using ReLU on the half of the neurons in the layer and the point reflection of ReLU on the other half.
% The same construction could be used with other ReLU family activation functions as well. 
% However, the focus of their work was to alleviate the need of normalizing layers and improve the performance of deep vanilla recurrent neural networks (RNNs) by using \emph{bipolar ReLU}.

% Both NCReLU and bipolar ReLU could have been used in the construction of a constrained neural network capable of representing non-convex functions, but to the best of our knowledge, they have not been so far.
%rebuttal
% The focus of attention when they were introduced was to increase performance of CNN networks on computer vision tasks and that was probably the reason why this, although important application, was overlooked.

%Learnable activation functions
%------------ Start of Figure. 

\begin{figure*}[!tp]
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/Unconstrained_ReLU25000_points.pdf}
        \caption{Unconstrained ReLU}
    \label{subfig:uncons_relu}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/Constrained_ReLU25000_points.pdf}
        \caption{Constrained ReLU}
        \label{subfig:cons_relu}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/Constrained_BiReLU25000_points.pdf}
        \caption{Constrained ReLU based activations}
        \label{subfig:cons_birelu}
    \end{subfigure}
    \hfill
    
    \caption{Approximations of the cubic function $f(x)=x^3$}
    \label{fig:example_prob}
\end{figure*}


% In recent years there has been a renovated interest in investigating activation function that can be learned during the training \citep{apicella2021}. In \cite{jin2016deep}, the authors propose \emph{S-shaped ReLU} learnable activation function able to learn both convex and non-convex monotone activation functions, a condition needed for building constrained monotonic neural networks as we will show below. Again, the authors' focus was on performance and suitability of this approach with respect to monotonocity was not discussed.
\subsection{Monotonicity by construction}

% Provided a monotone, non-decreasing activation function, a straightforward method to enforce non-decreasing monotonicity of a fully connected neural network is to constrain its weights to be non-negative as proposed in \cite{archer1993application}.
% moved below
% In \cite{daniels2010monotone}, authors prove the universal approximation property of constrained neural networks using sigmoid as the activation function: any multivariate continuous monotone function on a compact subset of $\mathbb{R}^k$ can be approximated with a constrained neural network of at most $k$ layers. 
% However, when compared to a neural network with a non-saturating activation function, the neural network using a saturating activation function (such as sigmoid and hyperbolic tangent) obtains inferior performance as shown in \cite{nair2010rectified, glorot2011deep}. This is also true in the case of constrained neural networks as described in the Section \ref{sec:experiments}. 

% If we replace sigmoid with a non-decreasing monotone convex activation function such as ReLU, resulting networks are easy to train and but can approximate convex functions only \citep{liu2020certified}. This limitation makes the method highly impractical as in the real-world use cases the functions modelled are rarely convex.


% In \cite{archer1993learning}, monotonicity is guaranteed by restricting the hypothesis space and by constraining the neural net weights to be positive. 
% In these works which ensure the (partial) monotonicity of outputs with respect to some or all of the inputs of a neural network by construction (more specifically by constrained weights) have a serious drawback- when used with modern, zero-centered monotonic activation functions such as ReLU or ELU, they can only approximate convex monotonic functions. Due to this shortcoming, the simple way of ensuring (partial) monotonicity by constraining weights does not perform well and is often not used in practice, but far more complex approaches to ensure monotonicity are used instead such as the methods proposed in  \cite{sivaraman2020counterexample, liu2020certified}.

Apart from the approaches mentioned in the introduction, another approach to building monotonic neural architecture is Min-Max networks where monotonic linear embedding and max-min-pooling are used \citep{sill1997monotonic}. In \cite{daniels2010monotone}, authors generalized this approach to handle functions that are partially monotonic and proved that the resulting networks have the universal approximation property. However, such networks are very difficult to train and not used in practice.


Deep lattice networks (DLN) \citep{you2017deep} use a combination of linear calibrators and lattices \citep{milani2016fast} for learning monotonic functions. This is the most widely used method in practice today, but not without its limits. Lattices are structurally rigid thereby restricting the hypothesis space significantly. They also require a very large number of parameters to obtain good performance.

% rebuttal
Given a model with a convex output function, it is possible to use backpropagation \cite{rumelhart1986learning} to make a monotonic model by computing the derivation of the output function. One simple way to construct a convex function is to use an unsaturated monotonic activation function in a fully connected layer as mentioned above or a more elaborate architecture such as the input convex neural networks \cite{pmlr-v70-amos17b}. These constructions are computationally more complex than the simple solution proposed here.


\subsection{Monotonicity by regularization}
Monotonicity can be enforced during the training by modifying the
loss function or adding a regularization term. 

In \cite{sill1996monotonicity}, the authors propose a modified loss function
that penalizes the non-monotonicity of the model. The algorithm models the input distribution as a joint Gaussian estimated from the training data and samples random pairs of monotonic points that are added to the training data. In \cite{gupta2019incorporate}, the authors propose a point-wise loss function that acts as a soft monotonicity constraint. These methods are straightforward to implement and can be used with any neural network architecture, but they do not guarantee the monotonicity of the trained model. 

Recently, there is an increasing number of proposed methods to certify or verify monotonicity obtained by regularization methods. In  \cite{liu2020certified}, the authors propose an optimization-based technique for mathematically verifying, or rejecting, the
monotonicity of an arbitrary piece-wise linear (e.g., ReLU) neural network. The method consists of transforming the monotonicity verification problem into a mixed integer linear programming (MILP) problem that can be solved using an off-the-shelf MILP solver.

In \cite{sivaraman2020counterexample}, the authors propose an approach that finds counterexamples (defined as the pair of points where the monotonicity constraint
is violated) by employing satisfiability modulo theories (SMT) solver \citep{barrett2018satisfiability}. To satisfy the monotonicity constraints, these counterexamples are included in the training data with adjustments to their target values to enforce the next iterations of the model to be monotonic.

Both methods \cite{liu2020certified,sivaraman2020counterexample} have been shown to support ReLU as the activation function only and there is no obvious way how to extend them to other activation functions. More precisely, they rely on piece-wise linearity of ReLU to work, the property not satisfied by other variants such as ELU, SELU, GELU, etc. Last but not least, the procedure for certifying/verifying using MILP or SMT solvers is computationally very costly. These approaches also require multiple reruns or iterations to arrive at certified/verified monotonic networks.

% \subsection{Universal approximation property}

% The classical Universal Approximation Theorem \citep{Cybenko1989,hornik1991,pinkus1999} states that any continuous function on a closed interval can be approximated with a feed-forward neural network with one hidden layer if and only if its activation function is nonpolynomial. In \cite{kidger2020}, authors prove the approximation property holds for arbitrary \emph{deep} neural networks with bounded number of neurons in each layer holds if the activation function is nonaffine and differential at at least one point.

% In \cite{daniels2010monotone}, authors shows the universal approximation property for constrained multivariate neural networks using \emph{sigmoid} as the activation functions: any multivariate continuous monotone function on a compact subset of $\mathbb{R}^k$ can be approximated with a constrained neural network with the sigmoid activation function of at most $k$ layers.

% However, the universal approximation theorem does not hold for constrained neural networks using monotone convex non-saturated activation functions: the resulting model are convex and cannot approximate non-convex functions.
% We hypothesize the universal approximation property with respect to monotonic functions holds if both convex and concave monotone activation functions are used. 
% We might even prove this in this paper or postpone the proof for the next one. 



==> 3_construction.tex <==
%auto-ignore


\section{Constrained neural networks}





% \subsection{Motivation}

 %------------ Start of Figure. 
\begin{figure*}[!tp]
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/ReLU_based_activations.pdf}
        \caption{ReLU based activations}
    \label{subfig:activation_relu}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/ELU_based_activations.pdf}
        \caption{ELU based activations}
        \label{subfig:activation_elu}
    \end{subfigure}
    \hfill
    \begin{subfigure}[t]{0.32\textwidth}
        \includegraphics[width=\textwidth]{Images/SELU_based_activations.pdf}
        \caption{SELU based activations}
        \label{subfig:activation_selu}
    \end{subfigure}
    \hfill
    
    \caption{Activation functions construction}
    \label{fig:activations}
\end{figure*}
% As mentioned above, ReLU and most of its variants are unbounded, non-decreasing, convex monotone functions. When used in fully-connected, feed-forward neural works with at least one hidden layer and with unconstrained weights, they can approximate any continuous function \citep{Cybenko1989},etc.

%
% A feedforward neural network without any constraints and with non-polynomial activation function can approximate any continuous function on a compact subset. In order to incorporate monotonicity, the weights of the neural network would need to be constrained to be non-negative. 

Most of the commonly used activation functions such as ReLU, ELU, SELU, etc. are monotonically increasing zero-centred, convex, lower-bounded non-polynomial functions. When used in a fully-connected, feed-forward neural network with at least one hidden layer and with unconstrained weights, they can approximate any continuous function on a compact subset. The simplest way to construct a monotonic neural network is to constrain its weights when used in conjunction with a monotone activation function. However, when the activation function is convex as well, the constrained neural network is not able to approximate non-convex functions. 


To better illustrate this, and to propose a simple solution in this particular example, we refer the readers to Figure \ref{fig:example_prob} where the goal is to approximate a simple cubic function $x^3$ using a neural network with a single hidden layer with either $2$ or $32$ neurons and with ReLU activation. A cubic function is apt for our illustration since it is concave in the considered interval $[-1, 0]$ and convex in the interval $[0, 1]$:
\begin{itemize}
    \item [\ref{subfig:uncons_relu}.] An unconstrained ReLU network with $n$ neurons can approximate both concave and convex segments of the cubic function using at most $n+1$ piecewise linear segments. Increasing the number of neurons will provide a better fit with the function being approximated. Notice that even though the cubic function is monotone, there is no guarantee that the trained model will be monotone as well.
    
    \item [\ref{subfig:cons_relu}.] If we constrain the weights of the network to be non-negative while still employing ReLU activation, the resulting model is monotone and convex. We can no longer approximate non-convex segments such as the cubic function on $[-1, 0]$ in the figure, and increasing the number of neurons from $2$ to $32$ does not yield any significant improvement in the approximation.
    
    \item[\ref{subfig:cons_birelu}.] Our proposed solution uses a combination of three activation functions in the hidden layer in order to gain the ability to model non-convex, monotone continuous functions. Notice that increasing the number of neurons increases the number of piecewise linear segments to approximate the cubic function. The resulting network is monotone by construction even when trained on noisy data.
\end{itemize}

%------------------------------------------
The schematic block diagram of our proposed solution (which we refer to as Constrained Monotone Fully Connected Layer or Monotonic Dense Unit interchangeably) is shown in the figure Fig. \ref{fig:mono_dense}. The individual components of the proposed solution are defined and described in the subsequent subsection.

% As can be seen from the Figure \ref{subfig:uncons_relu}, an unconstrained ReLU network can approximate both concave and convex parts of the cubic function but monotonicty is not guaranteed. If we naively constrain only the weights to be non-negative and employ ReLU activation, we can see in Figure \ref{subfig:cons_relu} that such a network can only learn to approximate the convex part of the cubic function. Even increasing the number of neurons from $2$ to $32$ does not help the network to approximate the cubic function. Upon employing the proposed modification to the constrained networks, wherein we employ the ReLU activation function for half of the neurons and point-reflection of ReLU for the other half neurons, 
% along with the non-negative weight constraint for preserving monotonicity, 
% we see that the network is able to faithfully approximate both convex and non-convex parts of the cubic function as shown in Figure \ref{subfig:cons_birelu}. 

% In order to illustrate the problem, we refer the Figure \ref{fig:example_prob} showing approximations of the cubic function $f(x)=x^3$ on the interval $[-1, 1]$ using unconstrained and constrained fully-connected neural networks with one hidden layer with plain and bipolar ReLU as an activation function,
%----------------------------------



%--------- Figure Monotonic Dense Unit
\begin{figure*}[!tp]
    \centering
    \includegraphics[width=0.72\textwidth]{Images/tikz_MonoDense.pdf}
    \caption{Proposed Monotonic Dense Unit or Constrained Monotone Fully Connected Layer}
    % The input to the layer is one dimensional vector $\mathbf{x}$ with $n$ elements and the output is one dimensional vector $\mathbf{y}$ with $m$ elements. The layer is parameterized with kernel weights $\mathbf{W}$, a two-dimensional matrix with $n\times m$ elements, and one dimensional vector bias $\mathbf{b}$ with $m$ elements. The weights $\mathbf{W}$ are then constrained to obtain $\mathbf{W'}$
%  using the operation $|.|_{t}$ with the help of  $n$-dimensional monotonicity indicator vector $\mathbf{t}$. \emph{convex} function $\breve{\rho}$ is monotonically increasing and convex activation function (such as ReLU, ELU) and $\hat{\rho}$ is its point reflection. We employ an $m$-dimensional \emph{activation selector vector} $\mathbf{s} \in [0, 1]^m$ to obtain a \emph{combined activation function} $\rho^{\mathbf{s}}$ is a weighted sum of $\breve{\rho}$ and $\hat{\rho}$.  Thus the output $\mathbf{y}$ is then obtained by  $\mathbf{y} =\rho^{\mathbf{s}}(|\mathbf{W}|_{\mathbf{t}} \cdot \mathbf{x} + \mathbf{b})$}
    \label{fig:mono_dense}
\end{figure*}
\subsection{Constrained monotone fully connected layer}

We say that a multivariate function $f: \mathbb{R}^n \rightarrow \mathbb{R}$ is \emph{partially monotonically increasing with respect to $x_i$} if 
$$
x_i^0 > x_i^1 \Rightarrow f\left(x_1, \dots, x_i^0, \dots x_n\right) \geq f\left(x_1, \dots, x_i^1, \dots x_n\right).
$$
Similarly, $f$ is \emph{partially monotonically decreasing with respect to $x_i$} if 
$$x_i^0 > x_i^1 \Rightarrow f\left(x_1, \dots, x_i^0, \dots x_n\right) \leq f\left(x_1, \dots, x_i^1, \dots x_n\right).$$
A set $S \subseteq R$ is \emph{compact} if every sequence in $S$ has a subsequence that converges to a point in $S$. One can easily show that closed intervals $[a, b]$ are compact, and compact sets can be thought of as generalizations of such closed bounded intervals.

Our construction is preconditioned on a priori knowledge of (partial) monotonicity of a multivariate, multidimensional function $f$. Let $f: K \mapsto \mathbb{R}^m$ be defined on a compact segment $K \subseteq \mathbb{R}^n$. Then we define its $n$-dimensional \emph{monotonicity indicator vector} $\mathbf{t} = [t_1, \dots, t_n]$ element-wise as follows:
\begin{equation}
    t_j= \begin{cases}
      1 & \text{if }\cfrac{\partial f(\mathbf{x})_i} {\partial x_j} \geq 0 \medspace
    \text{for each } i \in \{1, \dots , m\}\\
      -1 & \text{if }\cfrac{\partial f(\mathbf{x})_i} {\partial x_j} \leq 0  \medspace
    \text{for each } i \in \{1, \dots , m\}\\
      0 & \text{otherwise}
    \end{cases} 
    \: 
\end{equation}

Given an $(m \times n)$-dimensional matrix $\mathbf{M}$ and $n$-dimensional monotonicity indicator vector $\mathbf{t}$, we define the operation $|.|_{t}$ assigning an $(m \times n)$-dimensional matrix $\mathbf{M'} = |\mathbf{M}|_{t}$ to $\mathbf{M}$ element-wise as follows:
\begin{equation}
\label{eq:enforce_sign}
    m'_{j,i}= \begin{cases}
      |m_{j,i}| & \text{if }t_i=1\\
      -|m_{j,i}| & \text{if }t_i=-1\\
      m_{j,i} & \text{otherwise}
    \end{cases}
\end{equation}
% for every $i \in \{1, \dots, n \}$, $j \in \{1, \dots, m \}$.



\begin{definition}[Constrained linear layer] \label{def:constraned_lin_layer}
% Let $\mathbf{W}$ be an $(m \times n)$-dimensional matrix, $\mathbf{x}$ an $n$-dimensional vector, $\mathbf{b}$ an $m$-dimensional vector and $\mathbf{h}$ an $m$-dimensional vector. Then the output $\mathbf{h}$ of the \emph{constrained linear layer} with monotonicity indicator vector $\mathbf{t}$, weights $\mathbf{W}$, biases $\mathbf{b}$ and input $\mathbf{x}$ is:
%rebuttal
% Let $\mathbf{W}$ be an $(m \times n)$-dimensional matrix, $\mathbf{x}$ an $n$-dimensional vector and $\mathbf{b}$ an $m$-dimensional vector. 
Let $\mathbf{W} \in \mathbb{R}^{n \times m}$, $\mathbf{t} \in \{-1, 0, 1\}^n$,  $\mathbf{x} \in \mathbb{R}^n$ and $\mathbf{b} \in \mathbb{R}^m$.
The output $\mathbf{h} \in \mathbb{R}^m$ of the \emph{constrained linear layer} with monotonicity indicator vector $\mathbf{t}$, weights $\mathbf{W}$, biases $\mathbf{b}$ and input $\mathbf{x}$ is:
\begin{equation} \label{eqn:constraned_lin_layer}
\mathbf{h} = |\mathbf{W^T}|_{\mathbf{t}} \cdot \mathbf{x} + \mathbf{b}
\end{equation}
\end{definition}

\begin{lemma} \label{lem:mono_linear}
For each $i \in \{1, \dots, n\}$ and $j \in \{1, \dots, m\}$ we have:
\begin{itemize}
    \item if $t_i = 1$, then $\cfrac{\partial{h_j}}{\partial{x_i}} \geq 0$, and
    \item if $t_i = -1$, then $\cfrac{\partial{h_j}}{\partial{x_i}} \leq 0$.
\end{itemize}
\end{lemma}
% \begin{proof}
% From $\cfrac{\partial{h_j}}{\partial{x_i}} = w'_{i, j}$ and equation \ref{eq:enforce_sign}.
% \end{proof}

We use $\breve{\mathcal{A}}$ to denote the set of all zero-centred, monotonically increasing, convex, lower-bounded functions.

\begin{definition}  
Let $\breve{\rho} \in \breve{\mathcal{A}}$. Then
\begin{align}\label{eq:activation_concave}
    \hat{\rho}(x) & = -\breve{\rho}(-x) \\
    \label{eq:activation_saturated}
    \tilde{\rho}(x) & = \begin{cases}
      \breve{\rho}(x+1)-\breve{\rho}(1) & \text{if }x < 0\\
      \hat{\rho}(x-1)+\breve{\rho}(1) & \text{otherwise}
    \end{cases} 
\end{align}
    
\end{definition}

The main idea of our construction is use of three zero-centred, monotonically increasing activation functions, each applied to a part of neurons in a layer:
\begin{itemize}
    \item the original activation function $\breve\rho \in \mathcal{A}$,
    
    \item \emph{concave} \emph{upper-bounded}  function $\breve\rho$, and
    
    \item \emph{bounded function} $\tilde{\rho}$.
\end{itemize}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Plots of such constructed activation functions for popular activation functions are given in Figure \ref{fig:activations}. Using only convex and concave activation functions is sufficient for approximating many functions such as the cubic function in Figure \ref{fig:example_prob}, but not for e.g. the sigmoid function. As we will show below, the saturated activation function is crucial for the universal property of our construction.

\begin{definition}[Combined activation function] \label{def:combined_activation_func}
Let $\breve{\rho} \in \breve{\mathcal{A}}$, $\mathbf{h} \in \mathbb{R}^m$ and $\mathbf{s}=(\breve{s}, \hat{s}, \tilde{s}) \in \mathbb{N}^3$ such that $\breve{s} + \hat{s} + \tilde{s} = m$. Then the output of the combined activation function $\rho^\mathbf{s}: \mathbb{R}^m \rightarrow \mathbb{R}^m$ is defined element-wise as follows:
\begin{equation}\label{eqn:combined_activaion}
    \rho^{\mathbf{s}}(\mathbf{h)}_j = \begin{cases}
        \breve{\rho}(h_j) & \text{if } j \leq \breve{s} \\
        \hat{\rho}(h_j) & \text{if } \breve{s} < j \leq \breve{s} + \hat{s} \\
        \tilde{\rho}(h_j) & \text{otherwise} 
    \end{cases}
\end{equation}
\end{definition}

\begin{lemma}  \label{lem:mono_activation}
Let $\mathbf{y} = \rho^{\mathbf{s}}(\mathbf{h})$. Then for each $j \in \{1, \dots, m\}$ we have $\cfrac{\partial{y_j}}{\partial{h_j}} \geq 0$. Moreover
\begin{itemize}
\item if $\mathbf{s} = (m, 0, 0)$, then $\rho^{\mathbf{s}}_j$ is convex; and

\item if $\mathbf{s} = (0, m, 0)$, then $\rho^{\mathbf{s}}_j$ is concave.
\end{itemize}
\end{lemma}

%------------ Start of Neural architecture type 1 Figure. 
\begin{figure*}[!tp]
\centering
% \begin{minipage}{68.0\linewidth}
    % \begin{subfigure}[t]{0.8\textwidth}
        \includegraphics[width=0.9\textwidth]{Images/Composition_of_Monotonic_Dense.pdf}
        \caption{Neural architecture type 1}
    \label{subfig:neural_type_1}
    % \end{subfigure}
    % \hfill
% \end{minipage}
\end{figure*}
%%%%%%%%%%%%%%%%




\begin{definition}[Monotone constrained fully connected layer] \label{def:monotone_layer}
Let $n, m \in \mathbb{N}$, $\breve{\rho}\in \breve{\mathcal{A}}$, $\mathbf{t} \in \{-1, 0, 1\}^n$, $\mathbf{s}=(\breve{s}, \hat{s}, \tilde{s}) \in \mathbb{N}^3$ such that $\breve{s} + \hat{s} + \tilde{s} = m$, $\mathbf{W} \in \mathbb{R}^{n \times m}$, $\mathbf{x} \in \mathbb{R}^n$ and $\mathbf{b} \in \mathbb{R}^m$.

Then the output $\mathbf{y}$ of the \emph{monotone constrained fully connected layer} with monotonicity indicator vector $\mathbf{t}$, weights $\mathbf{W}$, biases $\mathbf{b}$ and input $\mathbf{x}$ is
\begin{align} \label{eqn:monotone_layer}
    \mathbf{y} & = \rho^{\mathbf{s}}\left(|\mathbf{W^T}|_{\mathbf{t}} \cdot \mathbf{x} + \mathbf{b}\right)
\end{align}
\end{definition}

From Lemma \ref{lem:mono_linear} and \ref{lem:mono_activation} directly follows:
\begin{corollary}
For each $i \in \{1, \dots, n\}$, $j \in \{1, \dots, m\}$ we have:

% \begin{itemize}
%     \item if $t_i = 1$, then $\cfrac{\partial{y_j}}{\partial{x_i}} \geq 0$;
%     \item if $t_i = -1$, then $\cfrac{\partial{y_j}}{\partial{x_i}} \leq 0$;
%     \item if $\mathbf{s} = \mathbf{1}$, then $\mathbf{y}_j$ is convex; and
%     \item if $\mathbf{s} = \mathbf{0}$, then $\mathbf{y}_j$ is concave.
% \end{itemize}
\begin{itemize}
    \item if $t_i = 1$, then $\cfrac{\partial{y_j}}{\partial{x_i}} \geq 0$,
    
    \item if $t_i = -1$, then $\cfrac{\partial{y_j}}{\partial{x_i}} \leq 0$, 
    
    \item if $\mathbf{s} = (m, 0, 0)$, then $\mathbf{y}_j$ is convex; and

    \item if $\mathbf{s} = (0, m, 0)$, then $\mathbf{y}_j$ is concave.
    
\end{itemize}
\end{corollary}

On the layer level, we can control both monotonicity, convexity and concavity of the output with respect to chosen input variables. The following section discuss how we can use such layers to build practical neural networks with the same properties.


\subsection{Composing monotonic constrained dense layers}


As mentioned before, the main advantage of our proposed monotonic dense unit is its simplicity. We can build deep neural nets with different architectures by plugging in our monotonic dense blocks. Figures \ref{subfig:neural_type_1} and \ref{subfig:neural_type_2}  show two examples of neural architectures that can be built using the proposed monotonic dense block. 

The first example shown in the Figure \ref{subfig:neural_type_1}, corresponds to the standard MLP type of neural network architecture used in general, where each of the input features is concatenated to form one single input feature vector $\mathbf{x}$ and fed into the network, with the only difference being that instead of standard fully connected or dense layers, we employ monotonic dense units throughout. For the first (or input layer) layer, the indicator vector $\mathbf{t}$, is used to identify the monotonicity property of the input feature with respect to the output. Specifically, $\mathbf{t}$ is set to $1$ for those components in the input feature vector that are monotonically increasing and is set to $-1$ for those components that are monotonically decreasing and set to $0$ if the feature is non-monotonic. For the subsequent hidden layers, monotonic dense units with the indicator vector $\mathbf{t}$ always being set to $1$ are used in order to preserve monotonicity. Finally, depending on whether the problem at hand is a regression problem or a classification problem (or even a multi-task problem), an appropriate activation function (such as linear activation or sigmoid or softmax) to obtain the final output.



% Neural network architectures can contain both monotonic features and non-monotonic features in the input.  For non-monotonic feature, we can employ any kind of neural network layer such as simple fully connected or dense layer, or embedding neural network layer or even complicated block such as transformer etc. For the sake of simplicity, we show neural architecture example with only dense layers. For monotonic feature, we specifically employ the proposed monotonic dense unit. It should be noted that our proposed monotonic dense unit would act as a regular dense layer without any constraint on weights if the indicator vector $\mathbf{t}$ is $0$. In this specific example, there is only one hidden monotonic dense layer and the bipolar activation is used in the hidden layer.  For the final output monotonic dense layer we do not employ any activation but only the weights are constrained to be non-negative to preserve monotonicity. 




%%Rebuttal

Figure \ref{subfig:neural_type_2} shows another example of a neural network architecture that can be built employing proposed monotonic dense blocks. The difference when compared to the architecture described above lies in the way input features are fed into the hidden layers of neural network architecture. Instead of concatenating the features directly, this architecture provides flexibility to employ any form of complex feature extractors for the non-monotonic features and use the extracted feature vectors as inputs. Another difference is that each monotonic input is passed through separate monotonic dense units. This provides an advantage since depending on whether the input is completely concave or convex or both, we can adjust the activation selection vector $\mathbf{s}$ appropriately along with an appropriate value for the indicator vector $\mathbf{t}$. Thus, each of the monotonic input features has a separate monotonic dense layer associated with it. Thus as the major difference to the above-mentioned architecture, we concatenate the feature vectors instead of concatenating the inputs directly. The subsequent parts of the network are similar to the architecture described above wherein for the rest of the hidden monotonic dense units, the indicator vector $\mathbf{t}$ is always set to $1$ to preserve monotonicity.




%------------ Start of Neural architecture type2 2Figure. 
\begin{figure*}[!tp]
\centering
% \begin{minipage}{68.0\linewidth}
    % \begin{subfigure}[t]{0.8\textwidth}
        \includegraphics[width=0.95\textwidth]{Images/Composition_of_Monotonic_Dense2.pdf}
        \caption{Neural architecture type 2}
    \label{subfig:neural_type_2}
    % \end{subfigure}
    % \hfill
% \end{minipage}
\end{figure*}


%------------ End of Neural architecture types Figure. 
% \subsection{Constrained monotone fully connected network}

% A monotonic deep neural network is constructed entirely by composition of monotone constrained fully connected (or dense) layers:


% \begin{definition}[Monotone constrained fully-connected neural network]
% Let $n$ and $m_1, \dots, m_k$ be positive natural numbers,  $\breve{\rho}$ a monotonically increasing \emph{convex} function, $\varrho$ a monotonically increasing function, $\mathbf{t}$ an $n$-dimensional monotonicity activation vector and $\mathbf{S} = (\mathbf{s}_1, \dots \mathbf{s}_{k-1})$ a tuple of selector weights vectors with dimensions $m_1, \dots, m_{k-1}$. Then the \emph{monotone constrained fully connected network} with $k$-layers, denoted $\mathcal{MFCN}_{\breve{\rho}, \mathbf{S}, \mathbf{t}, \varrho}$, is a tuple of monotone constrained fully connected layers and its final activation function $\varrho$:
% $$
% \mathcal{MFCN}_{\breve{\rho}, \mathbf{S}, \mathbf{t}, \varrho} = (\mathcal{MFC}_{\breve{\rho}, \mathbf{s}_1, \mathbf{t}}, \mathcal{MFC}_{\breve{\rho}, \mathbf{s}_2, \mathbf{1}}, \dots, \mathcal{MFC}_{\breve{\rho}, \mathbf{s}_{k-1}, \mathbf{1}}, \mathcal{MFC}_{\varrho, \mathbf{1}, \mathrm{id}}, \varrho)
% $$

% Moreover, let $\mathbf{W} = \mathbf{W}_1, \dots, \mathbf{W}_k$ be weights and $\mathbf{b} = \mathbf{b}_1, \dots, \mathbf{b}_k$ biases for the corresponding layers of $\mathcal{MFCN}_{\breve{\rho}, \mathbf{S}, \mathbf{t}, \varrho}$. Then the \emph{output function} of the monotone constrained fully connected network is the functional composition of the output functions of its layers and its final activation function:

% \begin{align}
%     \mathcal{MFCN}_{\breve{\rho}, \mathbf{S}, \mathbf{t}, \varrho}^{\mathbf{W}, \mathbf{b}} = \mathcal{MFC}_{\breve{\rho}, \mathbf{s}_1, \mathbf{t}}^{\mathbf{W}_1, \mathbf{b}_1} \circ \mathcal{MFC}_{\breve{\rho}, \mathbf{s}_2, \mathbf{1}}^{\mathbf{W}_2, \mathbf{b}_2} \circ \dots \circ \mathcal{MFC}_{\breve{\rho}, \mathbf{s}_{k-1}, \mathbf{1}}^{\mathbf{W}_{k-1}, \mathbf{b}_{k-1}} \circ \mathcal{MFC}_{\mathrm{id}, \mathbf{1}, \mathbf{1}}^{\mathbf{W_k}, \mathbf{b_k}}  \circ \rho
% \end{align}
% \end{definition}
% \hspace{1cm}

% \begin{lemma}
% Let $y=\mathcal{MFCN}_{\breve{\rho}, \mathbf{S}, \mathbf{t}, \rho}^{n, \mathbf{m}}(\mathbf{W_1}, \dots, \mathbf{W_k}, \mathbf{b_1}, \dots,  \mathbf{b_k},  \mathbf{x})$ for some weights $\mathbf{W_1}, \dots, \mathbf{W_k}$ and biases $\mathbf{b_1}, \dots,  \mathbf{b_k}$ and let $\rho$ be monotonically increasing function. For each $i \in \{1, \dots, n\}$ we have:
% \begin{itemize}
%     \item if $t_i = 1$, then $\cfrac{\partial{y}}{\partial{x_i}} \geq 0$;
%     \item if $t_i = -1$, then $\cfrac{\partial{y}}{\partial{x_i}} \leq 0$;
%     \item if $\mathbf{S} = \mathbf{1}$ and $\rho$ is convex, then $\mathbf{y}$ is convex; and
%     \item if $\mathbf{S} = \mathbf{0}$ and $\rho$ is concave, then $\mathbf{y}$ is concave.
% \end{itemize}
% \end{lemma}

% \subsection{Practical construction (old)}

% The schematic block diagram of our proposed monotonic dense unit is shown in the figure Fig. \ref{fig:mono_dense}.
% The input to the layer is one dimensional vector $\mathbf{x}$ with $n$ elements and the output is one dimensional vector $\mathbf{y}$ with $m$ elements. The layer is parametrized with kernel weights $\mathbf{W}$, a two-dimensional matrix with $n\times m$
%  elements, and one dimensional vector bias $\mathbf{b}$ with $m$ elements. The non-linear activation function $a(.)$ of a layer is mapping real values to real values. Typically, zero centered, monotonic functions such as ReLU and ELU are used. In the output layer of a network, we can also use sigmoid and softmax activation functions to output predicted probabilities. In such cases, we would use the original activation function instead of the weighted sum of activation function and its mirror.
% In practice, we often know that all output values are monotonic with respect to some, but not necessarily all, of the inputs. We express such knowledge with one dimensional monotonicity indicator vector $\mathbf{t}$ with $n$ elements. Concretely, we set $\mathbf{t}$ as follows:

% \begin{equation}
%     t_i= \begin{cases}
%       1 & \text{if $\frac{\partial y_j} {\partial x_i} \leq 0$}\\
%       -1 & \text{if $\frac{\partial y_j} {\partial x_i} > 0$} \\
%       0 & \text{otherwise}
%     \end{cases} 
%     \: \medspace
%     \text{for each $j \in 1, \dots , m$}
% \end{equation}


% Next, we enforce signs for layer weights depending on the value of indicator vector $\mathbf{t}$ with $n$ elements $t_1, \dots, t_n$, with each $t_i$ one with value $-1$, $0$ or $1$. The modified weights $\mathbf{W'}$ are calculated as a result of $enforce\_sign$ operation on  kernel weights $\mathbf{W}$ and with sign dependant on the value of indicator vector $\mathbf{t}$ as follows:


% \begin{equation}
%     \mathbf{W'} = enforce\_sign(\mathbf{W}, \mathbf{t)}
% \end{equation}

% More specifically, we have:
% \begin{equation}
%     w'_{i,j}= \begin{cases}
%       \mathrm{abs}(w_{i,j}) & \text{if $t=1$}\\
%       -\mathrm{abs}(w_{i,j}) & \text{if $t=-1$}\\
%       w_{i,j} & \text{if $t=0$}
%     \end{cases} 
%     \: \medspace
%     % \text{for each $j \in 1, \dots , m$}
% \end{equation}
% for each $i \in 1, \dots , n$ and $j \in 1, \dots , m$.


% The intermediate output vector $\mathbf{h}$ is then calculated by multiplying $\mathbf{W'}$ with the input vector $\mathbf{x}$ and adding with bias vector $\mathbf{b}$:
% \begin{equation}
%     \mathbf{h} = \mathbf{W'}\cdot\mathbf{x} + \mathbf{b}
% \end{equation}

% Next, a non linear activation function needs to be applied to the vector $\mathbf{h}$. Instead of a zero centered, monotonic activation function $a(h_j)$, we use a weighted sum of a with its point reflected or mirror function $-a(-h_j)$. We use an activation selector weight vector $\mathbf{s}$ with $m$ elements $s_1, s_2, \dots, s_m$ and calculate the output vector $\mathbf{y}$ as follows:
% \begin{equation}
%     \mathbf{y} = \mathbf{s}\cdot a(\mathbf{h}) + (1-\mathbf{s})\cdot (-a(-\mathbf{h}))
% \end{equation}
% The equation above employs element wise multiplication of vectors. This construction enables the network to learn both concave and convex shaped monotonic functions, or any combination of it. 
% Also, it should be noted that we can also employ two different activation functions $a_1(.)$ and $a_2(.)$ instead of the same activation function $a(.)$ with the only constraint being that both $a_1(.)$ and $a_2(.)$ activation functions should be  zero centered and monotonic activation functions. The resulting equation for output vector $\mathbf{y}$ then becomes:
% \begin{equation}
%     \mathbf{y} = \mathbf{s}\cdot a_1(\mathbf{h}) + (1-\mathbf{s})\cdot (-a_2(-\mathbf{h}))
% \end{equation}
% Some of the examples for activation functions that can be used are- ReLU, ELU, SELU, LeakyReLU, SoftPlus. We can either pair the activation functions with themselves (for example- $a_1(.) = a_2(.) = a(.) =$ ELU)  or we can pair two different activation functions (for example- $a_1(.) =$ ReLU, $a_1(.) =$ SELU) from the examples listed above.

% Finally, there is an important task of choosing the weighting vector $\mathbf{s}$. The activation selector weight  vector $\mathbf{s}$ is a one dimensional vector with $m$ elements and can be obtained by defining it at the time of network construction and the values are set based on the following: 
% % \begin{itemize}
%     % \item 
%     % $\mathbf{s}$ can be predefined at network construction time as one dimensional vector with $m$ elements where:
%     \begin{enumerate}
%         \item if the output is known to be fully convex, the vector is set to all ones
%         \item if the output is known to be  fully concave, the vector is set to all zeros, 
%         \item otherwise, some of the elements of the vector $\mathbf{s}$ are set to $1$ and the rest of the elements to $0$. We introduce a factor denoted by $\epsilon$ which indicates the fraction of elements of vector $\mathbf{s}$ to be set to $1$.  This fraction of elements being set to $1$ or set to $0$ can be a variable of our choice. For example, a straightforward approach is to set half of the values of  elements of vector s to 1 and the rest to 0 and the factor $\epsilon$ in this case is 0.5, and this would result in bipolar activation function. 
%     \end{enumerate}
%     In practice, we employ a convexity indicator vector $\mathbf{c}$ to set the vector $\mathbf{s}$ to ones or zeros or combination of them accordingly.
    
    % Future work and conclusion
    % \item Todo:Remove below :optimal values for each of the elements in vector $\mathbf{s}$ can be obtained from a learning scheme. One such scheme used in our proposed system uses auxiliary learnable weights $w_{s_1},\dots, w_{s_m}$ to calculate $s_1,\dots, s_m$ as follows:
    % \begin{equation}
    %     s_i = \sigma(w_{s_i})
    % \end{equation}
    % where $\sigma(.)$ is the sigmoid function.
% \end{itemize}
%------------- End of Subsection 

%--- Experiments on Learnable Activation

%% TODO: add proof

% \subsection{Universal approximation}

% We will use neural network layers with heterogeneous activation function sets etc.

% \begin{proposition}
% Let $\check{\rho}, \hat{\rho}: \mathbb{R} \to \mathbb{R}$ be monotone non-decreasing continuous non-polynomial functions and additionally let $\check{\rho}$ be convex and $\hat{\rho}$ be concave. Let $\mathcal{N}^{P}_n$ represent the class of feedforward neural networks with $n$ neurons in the input layer, one neuron in the output layer, and a single hidden layer with an arbitrary number of neurons, each one using an activation function from the set of possible activation functions $P$. Let $K \subseteq \mathbb{R}$ be compact. Then:
% \begin{itemize}
%     \item every $m \in \mathcal{N}^{\{ \check{\rho}, \hat{\rho} \}}_n \cup \mathcal{N}^{\{ \check{\rho}\}}_n \cup \mathcal{N}^{\{ \hat{\rho}\}}_n$ is a non-decreasing, monotone,  continuous function; 

%     \item every $m \in \mathcal{N}^{\check{\rho}}_n$ is convex; and

%     \item every $m \in \mathcal{N}^{\hat{\rho}}_n$ is concave.
% \end{itemize}
% Moreover, the following holds:
% \begin{itemize}
%     \item $\mathcal{N}^{\{ \check{\rho}, \hat{\rho} \}}_n $ is dense in the class of monotone functions $\mathcal{M}(K)$,
%     \item $\mathcal{N}^{\check{\rho}}_n $ is dense in the class of convex monotone functions $\acute{\mathcal{M}}(K)$,

%     \item $\mathcal{N}^{\hat{\rho}}_n $ is dense in the class of concave monotone functions $\grave{\mathcal{M}}(K)$,
% \end{itemize}  

% \end{proposition}

%%%%%%%%%%%%
%% This was done by me (Sharath), hence commenting
% \subsection{Notation and definitions}\label{sec:notation}
% We represent vectors with lowercase boldface letters, \eg $\mathbf{x}$, and matrices with uppercase boldface letters, \eg $\mathbf{W}$. Elements of vectors and matrices are denoted with lowercase subscripts. The $i-th$

% element of vector $\mathbf{x}$ is $x_i$ and the element in row $i$ and column $j$ of matrix $\mathbf{W}$ is $W_{ij}$.
% Given a function $\mathbf{y}=f(\mathbf{x})$, we denote by $\frac{\partial y_i}{\partial x_j}$ the partial derivative of the $i$-th component of $\mathbf{y}$ \wrt the $j$-th component of $\mathbf{x}$.

% In this work we focus on multilayer perceptrons (MLPs). Let the 
% function $\mathbf{y}=f(\mathbf{x})$ implement a MLP with $L+1$ layers. We denote a layer $k$ of the network by $\mathbf{h}^{(k)}$ for $k=0, \dots , L$. In particular, the input $\mathbf{x}$ and the output $\mathbf{y}$ correspond, respectively, to $\mathbf{h}^{(0)}$ and $\mathbf{h}^{(L)}$. As is customary, we represent a nonlinearity as $\sigma(\cdot)$. We can therefore write $\mathbf{h}^{(k+1)} = \sigma(\mathbf{W}^{(k)}\mathbf{h}^{(k)} + \mathbf{b}^{(k)})$, where $\mathbf{W}^{(k)}$ is the weight matrix and $\mathbf{b}^{(k)}$ is the bias. \par
% %
% Since there are multiple ways of defining an order in $\mathbb{R}^n$, we shall clarify which notion of monotonicity we are working with.

% \begin{definition}\label{def:mono_multi}
% A function $f: \mathbb{R}^n \rightarrow \mathbb{R}$ is called \textbf{monotonically increasing} (or non-decreasing) if for all $i=1,\dots,n$ the (univariate) restriction $f\mid_{i}: x_i  \mapsto y = f(\tilde{x}_1,\dots,x_i,\dots,\tilde{x}_n)$, obtained by fixing all the components except  the $i$-th, is monotonically increasing for every fixed value $\tilde{x}_j$ $\forall j = 1,\dots,n$ and $j\neq i$, in the usual sense of monotonicity for univariate functions. The definition for monotonically decreasing functions is analogous.
% \end{definition}
% %Define on closed subset
% %Merge into one

% %\mrm{in the above definition, is restriction the correct word? look at this page \url{https://math.stackexchange.com/questions/1198373/monotonicity-of-function-of-two-variables}. they have defined the same concept in a rather simple manner. }

% \begin{definition}\label{def:mono_multi_multi}
% A multivalued function $f: \mathbb{R}^n \rightarrow \mathbb{R}^m$ is called \textbf{monotonically increasing} if every component $f_i$ with $i = 1,\dots,m$ is monotonic according to Definition~\ref{def:mono_multi}.
% \end{definition}

% \section{Monotonic Features}\label{sec:mono_feat}
% Suppose that we want to interpret the prediction of an MLP with $L+1$ layers \wrt its $k$-th layer. In this section we present a way to constrain the $N^{(k)}$ units of the chosen interpretable layer $\mathbf{h}^{(k)} \in \mathbb{R}^{N^{(k)}}$ to be monotonic \wrt the units of the output layer $\mathbf{y} \in \mathbb{R}^{N^{(L)}}$. As mentioned before, in this work we focus only on MLPs. However, our strategy can be easily extended to different architectures. We refer to our neural network model with monotonicity constraints as \emph{MonoNet}.

% \subsection{Monotonically increasing layers}\label{sec:exp_layers}
% The first step in our construction is building monotonically increasing  layers. We follow the same idea as in \cite{daniels2010monotone, sill1997monotonic}. As discussed in \ref{sec:notation}, the $\mathbf{h}^{(k+1)}$ layer can be computed from the elements of layer  $\mathbf{h}^{(k)}$  as  $\mathbf{h}^{(k+1)} = \sigma(\mathbf{W}^{(k)}\mathbf{h}^{(k)} + \mathbf{b}^{(k)})$. We can now compute the partial derivatives of this relationship as:
% %
% \begin{equation}\label{eq:partial_der}
% \frac{\partial h^{(k+1)}_i}{\partial h^{(k)}_j} = \underbrace{\sigma'\Big(\sum_{t=1}^{N^{(k)}}W^{(k)}_{it}h^{(k)}_t + b^{(k)}_i\Big)}_{\geq 0}W^{(k)}_{ij}.
% \end{equation}
% %

% The most commonly used nonlinearities are non-decreasing functions, whose derivatives are always non-negative. Hence, the partial derivative in (\ref{eq:partial_der}) will be non-negative if and only if $W^{(k)}_{ij} \geq 0$. That is, $\mathbf{h}^{(k+1)}$ will be monotonically non-decreasing \wrt $\mathbf{h}^{(k)}$ if and only if the weight matrix has only non-negative entries. A way to impose this constraint is to apply to the weights a function with range in the positive numbers, such as the exponential function:
% \begin{equation}\label{eq:exp_layers}
%     \mathbf{h}^{(k+1)} = \sigma \Big(\mathrm{exp}(\mathbf{W}^{(k)})\mathbf{h}^{(k)} + \mathbf{b}^{(k)}\Big).
% \end{equation}
% Since the compositions of monotonically non-decreasing functions are also monotonically non-decreasing, we are guaranteed that, by stacking such layers, the last layer $\mathbf{y} = \mathbf{h}^{(L)}$ is monotonically non-decreasing \wrt the interpretable layer $\mathbf{h}^{(k)}$.\par
% %

% \subsection{Allowing arbitrary monotonicity}\label{sec:any_mono}

% The construction in the previous section enabled us to ensure a monotonically non-decreasing relationship between a chosen interpretable layer and the output. However, we would like \emph{each} component of the interpretable layer $\mathbf{h}^{(k)}$ to have an \emph{arbitrary} monotonic behavior (\ie either increasing or decreasing) \wrt \emph{each} component of the output $\mathbf{y}$. This can be achieved by component-wise rescaling of both $\mathbf{h}^{(k)}$ and $\mathbf{y}$. To see this let us introduce the auxiliary layers $\mathbf{\tilde{h}}^{(k)}$ and $\mathbf{\tilde{y}}$ so that
% \begin{equation}
%     \mathbf{\tilde{h}}^{(k)} = \boldsymbol{\alpha}\odot\mathbf{h}^{(k)}, \;\; \mathbf{y} = \boldsymbol{\beta}\odot\mathbf{\tilde{y}},
% \end{equation}

% where $\boldsymbol{\alpha} \in \mathbb{R}^{N^{(k)}}$, $\boldsymbol{\beta} \in \mathbb{R}^{N^{(L)}}$, and $\odot$ denotes a component-wise multiplication. If we stack monotonic layers from $\mathbf{\tilde{h}}^{(k)}$ to $\mathbf{\tilde{y}}$ as explained in Section~\ref{sec:exp_layers}, we find that the partial derivatives are
% \begin{equation}\label{eq:any_mono_der}
%     \frac{\partial h_i}{\partial y_j} = \underbrace{\frac{\partial \tilde{h}_i}{\partial \tilde{y}_j}}_{\geq 0} \frac{1}{\alpha_i \beta_j},
% \end{equation}
%  where the partial derivatives in terms of the auxiliary layers are positive. \par
 
 
 %rebuttal
\subsection{Universal approximation}

The classical Universal Approximation Theorem \citep{Cybenko1989,hornik1991,pinkus1999} states that any continuous function on a closed interval can be approximated with a feed-forward neural network with one hidden layer if and only if its activation function is nonpolynomial. In \citep{kidger2020}, authors prove the approximation property holds for arbitrary \emph{deep} neural networks with bounded number of neurons in each layer holds if the activation function is nonaffine and differential at at least one point.

In \cite{daniels2010monotone}, authors show the universal approximation property for constrained multivariate neural networks using \emph{sigmoid} as the activation functions: any multivariate continuous monotone function on a compact subset of $\mathbb{R}^k$ can be approximated with a constrained neural network with the sigmoid activation function of at most $k$ layers (Theorem 3.1), reproduced here for completeness:

\begin{theorem}\label{thm:universal_sigmoid}
For any continuous monotone nondecreasing function $f: K \xrightarrow{} \mathbb{R}$, where $K$  is a compact subset of $\mathbb{R}^k$, there exists a feedforward neural network using the sigmoid as the activation function with at most $k$ hidden layers, positive weights, and output $O$  such that $|O_x - f(x) | < \epsilon$, for any $x \in K$ and $\epsilon > 0$. 
\end{theorem}

However, the proof of the theorem uses only the fact that the Heavyside function $\mathbf{H}$ defined as
$$
H(x) = \left\{ \begin{array}{cc}
1     &  \textnormal{if } x\geq 0 \\
0     & \textnormal{otherwise}
\end{array} \right.
$$
can be approximated with the sigmoid function on a closed interval (since $\lim\limits_{a \to \infty} \sigma(a x) = H(x)$).

% It is important to note that this provides an upper bound on the number of monotonic layers in the general case and the number of layers for a particular function should be determined experimentally in practice (in our experiments in Section \ref{sec:experiments}, we got the best performing networks using 2-3 layers).

By construction, we have:
\begin{lemma}\label{lemma:heavyside_approx}
% Let $\breve{\rho} \in \breve{\mathcal{A}}$. Then the Heavyside function can be approximated with $\tilde{\rho}$ on a closed interval.
% \end{lemma}

% \begin{lemma}
Let $\breve{\rho} \in \breve{\mathcal{A}}$. Then the Heavyside function can be approximated with $\tilde{\rho}_H $ on $\mathbb{R}$, where
$$
\tilde{\rho}_H(x) = \alpha \tilde\rho(x) + \beta
$$
for some $\alpha, \beta \in \mathbb{R}$ and $\alpha > 0$.
\end{lemma}

\begin{lemma} \label{lemma:lin_comb_activation}
    Let $\tilde{\rho}_{\alpha, \beta}$ be an activation function for some $\alpha, \beta \in \mathbb{R}, \alpha>0$ such that for every $x \in \mathbb{R}$
    $$
        \tilde{\rho}_{\alpha, \beta}(x) = \alpha \tilde{\rho}(x) + \beta .
    $$
    Then for every constrained monotone neural network $\mathcal{N}_{\alpha, \beta}$ using $\tilde{\rho}_{\alpha, \beta}$ as an activation function ($s=(0, 0, \tilde{s})$), there is a constrained monotone neural network $\mathcal{N}$ using $\tilde{\rho}$ as an activation function such that for every $\mathbf{x} \in \mathbb{R}^{n}$:
    $$
        \mathcal{N}(\mathbf{x}) = \mathcal{N}_{\alpha, \beta}(\mathbf{x}) .
    $$
    
\end{lemma}

Finally, from Theorem \ref{thm:universal_sigmoid}, Lemma \ref{lemma:heavyside_approx} and Lemma \ref{lemma:lin_comb_activation}, we have the universal approximation property:

\begin{theorem}\label{thm:universal}
Let $\breve{\rho} \in \breve{\mathcal{A}}$. Then any multivariate continuous monotone function on a compact subset of $\mathbb{R}^k$ can be approximated with a monotone constrained neural network of at most $k$ layers using $\rho$ as the activation function.
\end{theorem}

The Theorem \ref{thm:universal} gives us the upper bound on the number of layers needed for approximating an arbitrary function. In practice, the number and width of layers for a given function and given dataset are found by hyperparameter search. The best results in our experiments were achieved by neural networks with a significantly smaller number of layers. The proof shows that the saturated activation functions are sufficient for the universal approximation property. However, experimental results show that the networks with predominately unsaturated activation functions are easier to train and achieve better results.



==> 4_experiment.tex <==
%auto-ignore

\section{Experiments}\label{sec:experiments}
 

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.3}
\small{
\begin{tabular}{l||rl|rl|rl}
\multirow{2}{*}{\bfseries Method} &
\multicolumn{2}{c|}{COMPAS}  &
\multicolumn{2}{c|}{Blog Feedback}  &
\multicolumn{2}{c}{Loan Defaulter} \\\cline{2-7}
   & Parameters & Test Acc $\uparrow$ &
  Parameters & RMSE $\downarrow$ 
& Parameters & Test Acc $\uparrow$ \\\hline
 Isotonic& N.A. & 67.6\% & N.A. & 0.203  & N.A. & 62.1\% \\
 XGBoost~\citep{xgboost} & N.A. & 68.5\% $\pm$ 0.1\%  & N.A. & 0.176 $\pm$ 0.005  & N.A. & 63.7\% $\pm$ 0.1\%\\
 Crystal~\citep{milani2016fast} & 25840 & 66.3\% $\pm$ 0.1\%  & 15840 & 0.164 $\pm$ 0.002 & 16940 & 65.0\% $\pm$ 0.1\% \\
 DLN~\citep{you2017deep}     & 31403 & 67.9\% $\pm$ 0.3\% & 27903 & 0.161 $\pm$ 0.001& 29949  & 65.1\% $\pm$ 0.2\% \\
 %Non-mono-DNN & 48451 & 68.2\% $\pm$ 0.2\%\\
 Min-Max Net~\citep{daniels2010monotone}     & 42000  & 67.8\% $\pm$ 0.1\% & 27700 & 0.163 $\pm$ 0.001  & 29000 & 64.9\% $\pm$ 0.1\%\\
  Non-Neg-DNN & 23112 & 67.3\% $\pm$ 0.9\% & 8492  & 0.168 $\pm$ 0.001 & 8502 & 65.1\% $\pm$ 0.1\%  \\
 Certified~\citep{liu2020certified} & 23112 & 68.8\% $\pm$ 0.2\%  & 8492 & 0.158 $\pm$ 0.001   & 8502 &  65.2\% $\pm$ 0.1\%  \\
 \textbf{Ours}    & \textbf{2317} & \textbf{69.2\% $\pm$ 0.2\%}& \textbf{1101} & \textbf{0.154 $\pm$ 0.001}   & \textbf{177} & \textbf{65.3\% $\pm$ 0.01\%} \\ 
\end{tabular}}
\vspace{5pt}
\caption{Comparison of our method with other methods described in \cite{liu2020certified}}
\label{tab:compas}
\end{table*}

\begin{table*}[htbp]
\centering
\setlength{\tabcolsep}{2pt}
\renewcommand\arraystretch{1.3}
\small{
\begin{tabular}{l||c|c}
\multirow{1}{*}{\bfseries Method} &
\multicolumn{1}{c|}{Auto MPG}  &
\multicolumn{1}{c}{Heart Disease} \\\cline{2-3}
& MSE $\downarrow$ 
 & Test Acc $\uparrow$ \\\hline
  Min-Max Net~\citep{daniels2010monotone}   & 10.14 $\pm$ 1.54  & 0.75 $\pm$ 0.04\\
 DLN~\citep{you2017deep} & 13.34  $\pm$ 2.42& 0.86 $\pm$ 0.02 \\
 COMET~\citep{sivaraman2020counterexample} & 8.81 $\pm$ 1.81  &  0.86 $\pm$ 0.03  \\
 \textbf{Ours}    & \textbf{8.37 $\pm$ 0.08}    & \textbf{0.89 $\pm$ 0.00} \\ 
\end{tabular}}
\vspace{5pt}
\caption{Comparison of our method with other methods described in \cite{sivaraman2020counterexample}}
\label{tab:comet}
\end{table*}
%  \subsection{Comparison with Other Methods}
In order to analyze the practical utility of the proposed method, we experiment with various datasets and compare them with the recent state-of-the-art. For the first set of experiments, we use the datasets employed by authors in \cite{liu2020certified} and use the exact train and test split for proper comparison. We perform experiments on 3 datasets: COMPAS~\citep{compas}, which is a classification dataset with 13 features of which 4 are monotonic; Blog Feedback Regression~\citep{buza2014feedback}, which is a regression dataset with 276 features of which 8  are monotonic; Loan Defaulter\footnote{https://www.kaggle.com/wendykan/lending-club-loan-data}, which is a classification dataset with 28 features of which 5 are monotonic. The dataset contains half a million data points. For comparison with other methods, we compare with \emph{Certified monotonic networks (Certified)} \cite{liu2020certified} and other methods described in it.

For the second set of experiments, we use 2 datasets: \emph{Auto MPG} (which is a regression dataset with 3 monotonic features) and \emph{Heart Disease} (which is a classification dataset with 2 monotonic features) as employed in the work \cite{sivaraman2020counterexample} and once again use the exact train and test split for proper comparison. We compare with the method \emph{COMET} described in \cite{sivaraman2020counterexample} along with \emph{Min-Max Net} \citep{daniels2010monotone} and \emph{Deep Lattice Network (DLN)} \citep{you2017deep} as described in  \cite{sivaraman2020counterexample}, and also more details regarding the datasets have been provided in the supplementary.
% \paragraph{Methods for Comparison:} We compare our method with six methods that can generate partially monotonic models. \emph{Isotonic Regression}: a deterministic method for monotonic regression~\citep{dykstra2012advances}. \emph{XGBoost}: a popular algorithm based on gradient boosting decision tree~\citep{xgboost}. \emph{Crystal}: an algorithm using ensemble of lattices~\citep{milani2016fast}. \emph{Deep Lattice Network (DLN)}: a deep network with ensemble of lattices layer~\citep{you2017deep}. 
% \emph{Non-Neg-DNN}: deep neural networks with non-negative weights. 
% \emph{Min-Max Net}: a classical three-layer network with one linear layer, one min-pooling layer, and one max-pooling layer~\citep{daniels2010monotone}.
 
%  \paragraph{Hyperparameter Validation:}  
 
We use cross-entropy for the classification tasks and we use mean-squared-error for the regression tasks as loss functions. We employ Bayesian optimization tuning with Gaussian process \cite{Snoek2012} to find the optimal hyperparameters such as the number of neurons, network depth or layers, initial learning rate etc.
 % For training, we first find the optimal learning rate using learning rate finder \cite{smith2017cyclical} and then train with one cycle policy \cite{smith2018disciplined}.

The code for experiments was written in the Keras framework \cite{chollet2015keras} and KerasTuner \cite{omalley2019kerastuner} via integration from the Tensorflow framework, version 2.11 \cite{tensorflow2015-whitepaper}. All experiments were performed using a Google Colaboratory instance with NVidia Tesla T4 GPU \cite{Bisong2019}. The code is publicly available at \cite{monocode}, while the preprocessed datasets for experiments are available at \cite{monodataset}.

%rebuttal
%The source code for all the experiments can be found at the following URL:\\
%\url{https://github.com/airtai/monotonic-dense-layer}
 
 \subsection{Results}\label{subsec:results}
The results for the datasets
above are summarized in Tables \ref{tab:compas} and \ref{tab:comet}. It shows that our method outperforms other methods in terms of test accuracy for classification tasks and mean squared error and root mean squared error (MSE and RMSE) for regression tasks. For each of the datasets, we run the experiments ten times after finding the optimal hyperparameters and report the mean and standard deviation of the best five results. Experiment results show that networks learned by our method can achieve better results with fewer parameters, than  
the best-known algorithms for monotonic neural networks, such as Min-Max Network~\citep{daniels2010monotone} and Deep Lattice Network~\citep{you2017deep}. It should be noted that the recent state-of-the-art works- \emph{Certified} \cite{liu2020certified} and \emph{COMET}  \cite{sivaraman2020counterexample} require multiple runs in order to even satisfy monotonic constraints whereas monotonicity is guaranteed by simply employing the proposed monotonic dense units. 

The most important advantage of our solution is simplicity and computational complexity. Our models have slightly better performance on all datasets we tested them on, but it is important to note they have significantly fewer parameters and the simplest training procedure. As such, they have the potential to significantly reduce the carbon footprint when used at scale:
\begin{itemize}
    \item The number of parameters of our model is an order or even two orders of magnitude smaller than alternatives. At prediction time, this translates roughly into 1-2 orders of magnitude less computation (most parameters are used in multiplications)

    \item At training time, we do not use any additional computationally expensive procedures apart from gradient descent, unlike alternative approaches such as \emph{COMET}  \cite{sivaraman2020counterexample} and \emph{Certified} \cite{liu2020certified}.

\end{itemize}



%rebuttal
% Finally, we made a number of experiments with more complex architectures which did not give any statistically relevant improvements in accuracy. One line of experiments were based on making the vector $s$ controlling convexity/concavity learnable. The resulting architecture was more difficult to train, sometimes getting stuck in a bad state. We also mixed different activation functions and/or their point reflections. The resulting architectures showed to advantage compared to the simple one.


==> 5_conclusion.tex <==
%auto-ignore

\section{Conclusion}

In this paper, we proposed a simple and elegant solution to build constrained monotonic networks which can approximate any continuous partially monotonic function. Specifically, we introduced a constrained monotone fully connected layer which can be used as a drop-in replacement for a fully connected layer to enforce monotonicity. We then employed our constrained monotone fully connected layer to build neural network models and showed that we can achieve better results to the recent state-of-the-art \cite{sivaraman2020counterexample, liu2020certified} in addition to the well-known works such as Min-Max networks \cite{daniels2010monotone} and DLNs \cite{you2017deep}. 
%rebuttal
However, the main advantage of the proposed solution is not higher accuracy but its computational and memory complexity: we use orders of magnitude fewer parameters and computation which makes the resulting neural networks more energy efficient. Last but not least, we proved such networks can approximate any multivariate monotonic function. 


% One drawback of our proposed method is that we are restricted by the choice of activation functions i.e., we can only employ monotonic activation functions. 

Extending these results to other types of neural network layers is straightforward, but we leave it for future work. E.g. convolutional layer can be made monotonic with respect to a subset of features by replacing its fully-connected filters with monotone constrained fully connected layers. As long as such layers are combined with other monotonic convolutional and fully connected layers and monotone activation functions, the resulting neural network would be monotone.
% We would like to investigate simple monotonic counterparts for other standard neural layers such as convolutional and recurrent neural networks and their variants, and attention models. 


% The main open question is can it approximate any monotonic function. It is easy to show that the universal approximation property holds for ReLU activation in case of a univariate continuous monotone function: the function can be approximated with a monotonic piecewise linear function, which can be easily constructed with a constrained neural network with one hidden layer in a way illustrated in Figure \ref{fig:example_prob}. We leave for future work extending the proof to activation functions other than ReLU and for the multivariate case.


==> 6_neuroips_checklist.tex <==
%auto-ignore

\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{} 
  \item Did you describe the limitations of your work?
    \answerYes{}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{In Appendix}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{Provided in supplementary} 
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{Provided as part of code in supplementary. Also, it should be noted that we build our experiments based on two previous state-of-the-arts - Certified Monotonic Network \cite{liu2020certified} and COMET \cite{sivaraman2020counterexample}, therefore for fair comparison, we employ the exact splits the authors employed in their repective works}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{See \ref{tab:compas}, \ref{tab:comet}}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Our code can be run on Google's Collaboratory and with default settings. A GPU instance uses a NVIDIA Tesla T4 GPU with 16GB RAM} 
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerNo{Our work has also been applied as patent.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{The code is included in the supplemental material and will be released on github}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

